Zero-shot Neural Transfer for Cross-lingual Entity Linking

Cross-lingual entity linking maps an entity mention in a source language to its corresponding entry in a structured knowledge base that is in a different (target) language. While previous work relies heavily on bilingual lexical resources to bridge the gap between the source and the target languages, these resources are scarce or unavailable for many low-resource languages. To address this problem, we investigate zero-shot cross-lingual entity linking, in which we assume no bilingual lexical resources are available in the source low-resource language. Specifically, we propose pivot-based entity linking, which leverages information from a high-resource "pivot" language to train character-level neural entity linking models that are transferred to the source low-resource language in a zero-shot manner. With experiments on 9 low-resource languages and transfer through a total of 54 languages, we show that our proposed pivot-based framework improves entity linking accuracy 17% (absolute) on average over the baseline systems, for the zero-shot scenario. Further, we also investigate the use of language-universal phonological representations which improves average accuracy (absolute) by 36% when transferring between languages that use different scripts.

==> old_files/data.tex <==
% \subsubsection{Data}
% \label{sec:data}

% \begin{table*}
%     \centering
%     \renewcommand{\arraystretch}{1.2}
%     \begin{tabular}{@{}lllllrr@{}}
%         \toprule
%          Source & Pivot & Lang. Family & Src. Script & Piv. Script & Coverage & Piv. Links \\\midrule
%          Uyghur (ug) & Turkish (tr) & Turkic & Arabic & Latin & 0.95 & 94K\\
%          Lao (lo) & Thai (th) & Tai--Kadai & Lao & Thai & 0.94 & 25K\\
%          Tigrinya (ti) & Amharic (am) & Afro--Asiatic & Ge'ez & Ge'ez  & 0.76 & 2K\\
%          Ukranian (uk) & Russian (ru) & Slavic & Cyrillic & Cyrillic & 0.74 & 316K\\
%          Javanese (jv) & Indonesian (id) & Austronesian & Latin & Latin & 0.72 & 87K\\
%          Uyghur (ug) & Uzbek (uz) & Turkic & Arabic & Latin & 0.65 & 72K\\
%          Punjabi (pa) & Hindi (hi) & Indo--Aryan & Gurmukhi & Devanagari & 0.59 & 21K\\
%          Telugu (te) & Tamil (ta) & Dravidian & Telugu & Tamil & 0.55 & 26K\\
%          Marathi (mr) & Hindi (hi) & Indo--Aryan & Devanagari & Devanagari & 0.42 & 21K\\
%          Bengali (bn) & Hindi (hi) & Indo--Aryan & Bengali & Devanagari & 0.36 & 21K\\\bottomrule
%     \end{tabular}
%     \caption{Data}
%     \label{tab:data}
% \end{table*}

% Table~\ref{tab:data} shows the different source-pivot language pairs we experiment with. We collect Wikipedia\footnote{\url{https://dumps.wikimedia.org}} article titles from each language and remove titles that are not named entities (locations, persons and organizations), based on DBPedia categories\footnote{\url{http://dbpedia.org}}. The information from Wikipedia has inter-language links for each title, which we use both as parallel data for training the max-margin encoder (Section~\ref{sec:encoder}) and as equivalent entities for pivoting (Section~\ref{sec:pivot}). The source-pivot pairs were selected based on several criteria:
% \smallskip

% {\parindent0pt
% \textbf{Wikipedia availability}.\quad The multilingual structured information on Wikipedia is ideal for testing our method. We choose source and pivot languages such that there exists a Wikipedia in both, but the source language Wikipedia has significantly fewer articles than the pivot.
% \smallskip

% \textbf{Conversion to IPA}.\quad We use Epitran\footnote{\url{https://github.com/dmort27/epitran}}, a tool for converting orthographic text to IPA. We ensure that our experimental languages are supported by Epitran, since we aim to compare EL with orthographic and phonological representations.
% \smallskip

% \textbf{Language family and written script}.\quad The pivot language is selected from the same language family as the source. We choose pairs from a wide variety of language families in order to test the universality of our model. We also ensure to test on some source-pivot pairs that use the same script as well as others that use different scripts.
% \smallskip

% \textbf{Source Wikipedia Coverage}.\quad We measure the fraction of named entities in the source Wikipedia that are also present in the pivot Wikipedia. Table~\ref{tab:data} shows that our selection of languages has a wide range of this coverage.

% }

% Table~\ref{tab:data} shows the number of inter-language links between the pivot and English Wikipedias. We randomly sample $10$K links for each pivot language (apart from \textit{am} for which we use the available $2$K) for creating a training set for the max-margin encoder. While pivoting, we use all available language links as mentioned in Table~\ref{tab:data}. 

% Our `gold-standard' test data is created using inter-language links between the source Wikipedia and English Wikipedia. We randomly choose $5$K entities for each test language, the exceptions being the particularly low-resource languages where we use all available entities. These are \textit{ti}, \textit{lo} and \textit{ug} with $90$, $579$ and $1297$ test examples respectively. 


% % \subsection{Wikipedia}
% % \subsection{LORELEI}

==> old_files/expold.tex <==
\section{Experiments}

\subsection{Baselines}
Existing work uses, at the very least, a lexicon in the source language to aid cross-lingual EL. For fair comparison to our method, we construct the following baselines that do not require any resources in the source language:

\gn{This needs to be re-written to reflect that we now have experiments on pivoting with \textsc{Exact} and \textsc{Translate}?}

\textsc{Exact}: We consider the entity link to be, if found, the exact string match of the entity in either the \textit{pivot} or the \textit{English} knowledge base. If there is no match, the link is considered incorrect.

\textsc{Translate}: We generate a bilingual lexicon with word alignments obtained from parallel Wikipedia titles and use word-by-word translation for entity linking, as described in~\citet{pan-EtAl:2017:Long2} \gn{How do you create the lexicon?}. With the lexicon, each word in the input entity is translated to English. The entity link is the exact match of the obtained translation, if found in the \textit{English} knowledge base. For fair comparison with our method, we use Wikipedia titles from the \textit{pivot language}, rather than the source language of the input entity.

\textsc{NoPivot}: We train a max-margin similarity encoder (Section~\ref{sec:encoder}) on parallel Wikipedia titles between the \textit{pivot language} and \textit{English}. In order to find the entity link, we use the \textit{pivot language} encoder to encode the input entity and select the English entity from the knowledge base with the highest cosine similarity (as encoded by the \textit{English} encoder). 

\subsection{Experiment Configuration}

\gn{Make sure that you have a table that shows the scripts, coverage, etc., for each setup.}

Train and validation sets, test sets, hyperparameters, evaluation metric

\begin{table*}
\centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lll|ccccccccccc}
% \toprule
  Model & In. & Piv. & ti-am & ug-uz & ug-tr & mr-hi & bn-hi & pa-hi & te-ta & ku-fa & jv-id & uk-ru & lo-th\\\midrule
  \multirow{2}{*}{\textsc{Exact}} & \multirow{2}{*}{G} & - & 0.02 & 0.03 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & \textbf{0.38} & 0.66 & 0.02 & 0.02 \\
   &  & + & 0.46 & 0.04  & 0.03  & 0.11 & 0.00 & 0.00 & 0.00 & 0.38 & 0.79  & 0.14 & 0.02   \\ \midrule
  \multirow{2}{*}{\textsc{Trans}} & \multirow{2}{*}{G} & - & 0.46 & 0.03 & 0.03 & 0.14 & 0.00 & 0.00 & 0.00 & 0.38 & 0.66 & 0.02 & 0.02 \\
  & & + & 0.47 & 0.04 & 0.03 & 0.16 & 0.00 & 0.00 & 0.00 & 0.38 & 0.79 & 0.14 & 0.02   \\ \midrule
  \multirow{6}{*}{\textsc{Encode}} & \multirow{2}{*}{G} & - & 0.46 & 0.05 & 0.06 & 0.48 & 0.00 & 0.00 & 0.00 & 0.38 & 0.74 & 0.22 & 0.02 \\
  & & + & 0.64 & 0.07 & 0.08 & 0.58 & 0.00 & 0.00 & 0.00 & 0.38 & \textbf{0.88} & \textbf{0.42} & 0.02 \\ \cmidrule{4-14}
   & \multirow{2}{*}{P} & - & 0.39 & 0.09 & 0.07 & 0.40 & 0.16 & 0.08 & 0.07 & 0.02 & 0.20 & 0.01 & 0.02 \\
  & & + & 0.66 & \textbf{0.18} & \textbf{0.14} & 0.52 & \textbf{0.20} & \textbf{0.12} & \textbf{0.11} & 0.03 & 0.40 & 0.16 & \textbf{0.22} \\\cmidrule{4-14}
   & \multirow{2}{*}{G+P} & - & 0.52 & 0.04 & 0.04 & 0.52 & 0.00 & 0.01 & 0.00 & 0.38 & 0.71 & 0.13 & 0.02 \\
  & & + & \textbf{0.68} & 0.06 & 0.05 & \textbf{0.61} & 0.01 & 0.01 & 0.00 & 0.38 & 0.87 & 0.28 & 0.02 \\
  
 \bottomrule
\end{tabular}
}
\caption{Entity linking accuracy for each model with \textbf{G}rapheme or \textbf{P}honeme input, and without (-) or with (+) pivoting. \gn{Multiple comments: (1) Are these in any particular order? I would try to choose a consistent and salient order such as decreasing pivot-language coverage. (2) For ku-fa, multiple settings tie, so all should be bold. Same for any others where there's a tie. (3) If time allows, we could measure statistical significance using Fisher's exact test or paired bootstrap resampling.}}
\label{table: results}
\end{table*}

\subsection{Results and Discussion}

\gn{These results seem to be divided into subsections in a slightly awkward way. Let me propose a slight re-structuring based on research questions. (1) ``Does the proposed max-margin method outperform previous work?'' Here we compare the first and third lines (baselines) with the others. (2) ``Is pivoting effective?'' Here we compare the pivoted models with unpivoted models. (3) ``What is the interplay of the input representation and language pair?'' I think that rearranging in this way might make things flow better.}

\gn{Also, we need qualitative examples. Maybe one for each of the research questions.}

Table~\ref{table: results} summarizes the entity linking accuracy for the baselines and our pivoting method. First, examining the utility of the pivoting method, we can see that it leads to higher accuracy than the respective baselines for all source-pivot language pairs, apart from Kurmanji-Farsi (\textit{ku-fa}) where no method is able to exceed the exact-match baseline 
\gn{It's a bit strange to me that we see \emph{no} improvement on ku-fa even though the exact match is so high. It seems that the grapheme encoder should do quite well. Do you have any idea what's happening here? The other results look reasonable I guess.}. The performance depend on how we represent the characters (graphemes or phonemes), as well as on the source-pivot language pair. We present a detailed analysis of each in the following sections.

\subsubsection{Performance of Baselines}

\gn{This sub-section needs to be re-written to match the current results. It might be better to split into a discussion of the utility of pivoting, vs. the utility of the max-margin encoder. Also, It might not be necessary to make this a separate subsection. It could potentially be included in the main results.}
The \textsc{Exact} and \textsc{Translate} methods fail in the phonetic space because these rely on exact string matches and having completely identical IPA for the same entity across languages is rare.
It can be seen that the \textsc{Exact} and \textsc{Translate} methods perform reasonably in the cases where the script used by the source and pivot languages are the same, as some portion of entities might be written exactly the same way. The high accuracy of the baselines for \textit{jv-id} and \textit{ku-fa} is explained by the fact that both these source languages are written in the Latin script -- since the KB is in the Latin script as well, string-lookup methods can easily lead to finding the correct entity link~\citep{TsaiRo18}.

The \textsc{NoPivot} baseline has lower accuracy as compared to the pivoting method for all languages. However, it is consistently competitive or better than the \textsc{Exact} and \textsc{Translate}, particularly with IPA representations, indicating that our encoder model can be used for EL even when there are no pivot-KB links available.


\subsubsection{Effect of Pivot Language}

The pivoting method performs extremely well for source-pivot languages that are closely related and have the same orthography. We see high accuracy for \textit{ti-am}, \textit{mr-hi}, \textit{jv-id} and \textit{uk-ru}. 

We note that our method performs poorly in the case of \textit{ku-fa}. While using graphemes, this is expected because Kurmanji (\textit{ku}) uses the Latin script, while Farsi (\textit{fa}) uses the Perso-Arabic alphabet. Since our KB is in English, an exact string match between \textit{ku} names and KB works better than our encoding method. In the phonetic space, we notice that although \textit{ku} and \textit{fa} belong to the same broad language family, entities seem to have largely different IPA representations. For example, the IPA for `Estonia' in \textit{fa} and \textit{ku }is \textipa{6stvnj} and \textipa{Estonja:} respectively. This hampers the performance of pivoting in the phonetic space.
%\gn{But why doesn't the encoder work at all? It seems that the non-pivoting encoder in Grapheme space should work, and the IPA encoder should have some effect as well.}\sr{ku and fa have different scripts so the grapheme encoder doesn't work here}\gn{Right, but what about for English? The non-pivoted model (which doesn't even use fa) should be able to match at least a few words in English.}\sr{we use the pivot language encoder to encode the mention in both cases}\gn{Ahh, right.} \sr{to be honest, i don't know why IPA doesn't work and I can't find references that state ku-fa are significantly different phonetically (just anecdotes on q/a forums)}\gn{What about sending your results to David and asking him to take a look?} \sr{will do}\gn{And also make sure that the answer to the question about why ku-fa is not working is clear here.}

For the other source-pivot pairs that differ in orthography, we see reasonable performance in the phonetic space. Using Uzbek (\textit{uz}) and Turkish (\textit{tr}) as transfer languages for Uyghur (\textit{ug}) leads to an increase in performance in the IPA space, similar to observations noted by~\citep{bharadwaj-EtAl:2016:EMNLP2016}. The same trend is observed with the Indic (\textit{bn-hi} and \textit{pa-hi}), the Dravidian (\textit{te-ta}) and the Tai–Kadai (\textit{lo-th}) language pairs.

Overall, our results show that the selection of an appropriate pivot language is paramount to the success of our method. We also note that having a large amount of parallel training data between the pivot language and the KB language is not necessary -- the pivoting method has high accuracy for \textit{ti-am} in both the orthographic and phonetic space, with less than $2300$ \textit{am-en} language links for training the encoder. 

\subsubsection{Character Representation}

We experiment with using grapheme and phoneme representations of the entities with our model. In Table~\ref{table: results}, we observe that using graphemes offers higher accuracy than phonemes in almost all cases where the source and pivot languages share orthography. However, the grapheme methods completely fail when the source and pivot languages use different scripts. Converting entities to the universal IPA space enable us to do EL across orthographies, and we note that the phoneme pivoting method shows convincing improvement over the baselines in these cases.

\todo{Grapheme+phoneme doesn't work the best: why?}

\subsubsection{Why Pivoting Helps}

The pivoting method improves on the accuracy of \textsc{NoPivot} for all the experimental settings (Table~\ref{table: results}). Naturally, pivoting can only be beneficial when the `correct' KB entry for a given mention is present in the pivot language KB as well. This could lead to the `correct' entry getting a higher score and being selected as the entity link.

On average, the accuracy for test mentions that have the appropriate link in the pivot KB increases by an absolute value of around $0.10$. For those mentions that do not have the correct link in the pivot KB, accuracy decreases by less than $0.01$ (absolute), averaged over all language pairs. This indicates that using a pivot language, in general, increases the EL accuracy while not affecting the test examples that the model already performs well on.
\todo{add this table to supplementary?}

\gn{I think up to here can be restructured according to my comment at the top.}

\begin{table}[]
    \centering
    \begin{tabular}{l|rrr}
         Pivot & LOC & PER & ORG \\\midrule
         - & 0.27 & 0.34 & 0.24 \\
         + & 0.37 & 0.39 & 0.32 \\
    \end{tabular}
    \caption{Average Entity Type EL Accuracy}
    \label{table:type_results}
\end{table}

\subsubsection{Results by Entity Type}

Table~\ref{table:type_results} details the average EL accuracy over all languages for each type of entity in our test set -- persons (PER), organizations (ORG) and locations (LOC). In general, we see that pivoting increases the accuracy for all entity types, more so for ORG and LOC.

ORG entities have a slightly lower overall accuracy than LOC and PER. This is likely because LOC and PER are most often loose transliterations across languages, but ORG names have function words that are translated across languages. The pivoting method seems to alleviate this problem to some extent. \todo{example of where pivoting works}

An anomaly in this case is the \textit{uk-ru} experiment, where the PER accuracy is significantly lower than the other entity types. This is likely because Wikipedia titles in \textit{ru} are ordered \textit{last name, first name} while in \textit{uk}, they are ordered \textit{first name, last name}. \todo{example}


\begin{table}
    \centering
    \begin{tabular}{c|c}
        Source-Pivot & Recall @20 \\\midrule
         ti-am & 0.74 \\ 
         ug-uz & 0.29 \\
         ug-tr & 0.21 \\
         mr-hi & 0.76 \\
         bn-hi & 0.39 \\
         pa-hi & 0.28 \\
         te-ta & 0.24 \\
         ku-fa & -- \\
         jv-id & 0.91 \\
         uk-ru & 0.63 \\
         lo-th & 0.35
         
    \end{tabular}
    \caption{Recall @20 Candidates \gn{Could you make this a graph with multiple data points instead? This ridiculously tall table is a bit awkward and doesn't seem to tell much.}}
    \label{table:candidate}
\end{table}


\subsubsection{Pivoting for Candidate Generation}

The EL process, in most existing work, is a two-step pipeline -- candidate generation and precise disambiguation~\citep{Hachey:2013:EEL:2405838.2405914}. Candidate generation serves to reduce the search-space for EL, by selecting a small number of candidates from a large KB for more precise linking. Selecting candidates is required because precise linking algorithms are often prohibitively expensive to use on the millions of entries in the KB.

Although a more precise linking step is not in the scope of our current work, we discuss how our pivoting method can be used for candidate generation. Table~\ref{table:candidate} shows the `Recall @20' -- the fraction of instances when the correct entity link is present in the top $20$ entities as scored by our system~\citep{TsaiRo18}. We use the best system for each language pair (Table~\ref{table: results}). For \textit{ku-fa}, the best system is \textsc{Exact}, which does not produce a scored list of candidates. The Recall @20 is high for several language pairs, particularly those that share orthography. Since the KB has over 2 million entries, our pivoting method can be an effective way to generate a smaller number of candidates to be used in a sophisticated disambiguation method for higher quality EL.


==> old_files/results.tex <==
\section{Results and Discussion}
\label{sec:results}

% \begin{table*}
% \centering
% \renewcommand{\arraystretch}{1.2}
% %\resizebox{\textwidth}{!}{
% \begin{tabular}{@{}lll|cccccccccc@{}}
% % \toprule
%   Model & In. & Piv. & ti-am & ug-uz & ug-tr & mr-hi & bn-hi & pa-hi & te-ta & jv-id & uk-ru & lo-th\\\midrule
%   \multirow{2}{*}{\textsc{Exact}} & \multirow{2}{*}{G} & - & 0.02 & 0.03 & 0.03 & 0.00 & 0.00 & 0.00 & 0.00 & 0.66 & 0.02 & 0.02 \\
%   &  & + & 0.46 & 0.04  & 0.03  & 0.11 & 0.00 & 0.00 & 0.00 & 0.79  & 0.14 & 0.02   \\ \midrule
%   \multirow{2}{*}{\textsc{Trans}} & \multirow{2}{*}{G} & - & 0.46 & 0.03 & 0.03 & 0.14 & 0.00 & 0.00 & 0.00  & 0.66 & 0.02 & 0.02 \\
%   & & + & 0.47 & 0.04 & 0.03 & 0.16 & 0.00 & 0.00 & 0.00 & 0.79 & 0.14 & 0.02   \\ \midrule
%   \multirow{6}{*}{\textsc{Encode}} & \multirow{2}{*}{G} & - & 0.46 & 0.05 & 0.06 & 0.48 & 0.00 & 0.00 & 0.00 & 0.74 & 0.22 & 0.02 \\
%   & & + & 0.64 & 0.07 & 0.10 & \textbf{0.58} & 0.00 & 0.00 & 0.00 & \textbf{0.88} & \textbf{0.42} & 0.02 \\ \cmidrule{4-13}
%   & \multirow{2}{*}{P} & - & 0.40 & 0.12 & 0.10 & 0.40 & 0.16 & 0.08 & 0.07 & 0.67 & 0.03 & 0.04 \\
%   & & + & \textbf{0.69} & \textbf{0.21} & \textbf{0.16} & 0.52 & \textbf{0.20} & \textbf{0.12} & \textbf{0.11} & 0.84 & 0.15 & \textbf{0.25} \\
  
%  \bottomrule
% \end{tabular}
% %}
% \caption{Entity linking accuracy for each model with \textbf{G}rapheme or \textbf{P}honeme input, and without (-) or with (+) pivoting. \gn{Multiple comments: (1) Are these in any particular order? I would try to choose a consistent and salient order such as decreasing pivot-language coverage. (2) For ku-fa, multiple settings tie, so all should be bold. Same for any others where there's a tie. (3) If time allows, we could measure statistical significance using Fisher's exact test or paired bootstrap resampling.}}
% \label{table: results}
% \end{table*}

Table~\ref{table: results} summarizes the entity linking accuracy for the baselines and our pivoting method. First, we can see that the proposed combination of the entity encoder and pivoting leads to higher accuracy than the respective baselines for all source-pivot language pairs. % We also note that performance depends on how we represent the characters (graphemes or phonemes).
In the following sections, we attempt to answer the following research questions: (1) ``Does the proposed max-margin encoding method outperform the baselines?'' (2) ``Is pivoting effective?'' (3) ``What is the interplay of the input representation and language pair?'' (4) ``What is the potential of using pivoting in the retrieval step in 2-step EL reranking systems?'' (5) ``How does unsupervised linking compare to when we have some small amount of supervised data?''

\subsection{Performance of \textsc{Encode}}

In this section, we analyze the performance of our max-margin encoder relative to the baselines, for both the non-pivot and pivot settings. 

In Table~\ref{table: results}, we see that the \textbf{--Piv.} \textsc{Exact} method performs well when $l_s$ is in Latin script as several entities are identical to their English counterparts~\citep{TsaiRo18}, i.e. with the \texttt{jv-id} language pair. For the other languages, the source mentions are not in the same script as English, which renders exact string matches impossible. The \textbf{--Piv.} \textsc{Translate} baseline performs reasonably well as the lexicon converts $m$ into an English string that can be matched with the KB. In the corresponding setting with \textsc{Encode}, we see the non-pivoting grapheme-based encoder performs as well or better than both the baselines for all language pairs. 

We attempted to use \textsc{Exact} and \textsc{Translate} in the phonetic space, but the accuracy was $\approx 0$ because having completely identical IPA across languages is rare and exact matching fails. The phoneme-based \textbf{--Piv.} \textsc{Encode} method outperforms the grapheme-based \textbf{--Piv.} model significantly when $l_s$ is not written in the Latin script.

Similar observations hold for the pivoting experiments. The \textbf{+Piv.} \textsc{Encode} baseline performs better than \textbf{+Piv.} \textsc{Exact} and \textbf{+Piv.} \textsc{Translate}, indicating that our encoder is able to transfer from $l_p$ to $l_s$ effectively. 

Note that \textbf{--Piv.} \textsc{Encode} is consistently competitive or better than the baselines, particularly with IPA representations, indicating that our encoder model can be used effectively even without pivoting. We also note that having a large amount of parallel data for training the encoder is not necessary; \textsc{Encode} obtains high accuracy for \texttt{ti-am} with less than $2300$ \texttt{am-en} training examples. 


\subsection{Utility of Pivoting}

\begin{figure}
    \centering
    \includegraphics[width=0.8\columnwidth]{acl18-latex/images/qual_ex.pdf}
    \caption{Examples of successes from our dataset}
    \label{fig:qual_ex}
\end{figure}

% \begin{table}[]
%     \centering
%     \begin{tabular}{@{}l|rrr@{}}
%          Pivot & LOC & PER & ORG \\\midrule
%          -- & 0.28 & 0.29 & 0.21 \\
%          + & 0.40 & 0.36 & 0.31 \\
%     \end{tabular}
%     \caption{Average Entity Type EL Accuracy}
%     \label{table:type_results}
% \end{table}

The pivoting method improves on the accuracy of \textbf{--Piv.} for all the experimental settings (Table~\ref{table: results}). In particular, \textbf{+Piv.} performs extremely well for source-pivot languages that have the same orthography (\texttt{ti-am}, \texttt{mr-hi}, \texttt{jv-id}, \texttt{uk-ru}). For the source-pivot pairs that differ in orthography, pivoting leads to performance increase in the phonetic space. Figure~\ref{fig:qual_ex} shows an example from our \texttt{jv} test dataset that is wrongly linked with \textbf{--Piv.}, but correctly linked when pivoting through \texttt{id}.   

Naturally, pivoting can only be beneficial when the `true' KB entity for mention $m$ is present in $\mathcal{E}_p$, which could lead to this entity getting a higher score and being selected as the entity link.

For the \textsc{Encode} model, the accuracy for test mentions that have the `true' link in $\mathcal{E}_p$ increases by an absolute value of around $10\%$ (averaged over all language pairs). For those mentions that do not have the `true' link in $\mathcal{E}_p$, the average accuracy decreases by less than $1\%$ (absolute). This indicates that pivoting, in general, increases the EL accuracy while not affecting the test examples that the model already performs well on.

% \textbf{Results by Entity Type}. Table~\ref{table:type_results} details the average EL accuracy over all languages for each type of entity in our test set -- persons (PER), organizations (ORG) and locations (LOC). In general, we see that pivoting increases the accuracy for all entity types, more so for ORG and LOC. ORG entities have a lower overall accuracy than LOC and PER. This is likely because LOC and PER are most often loose transliterations across languages, but ORG names have function words that are translated. The pivoting method seems to alleviate this problem to some extent. \todo{example of where pivoting works}

